A Polynomial Kernel for Proper Helly Circular-arc Vertex Deletion

A proper Helly circular-arc graph is an intersection graph of a set of arcs on a circle such that none of the arcs properly contains any other arc and every set of pairwise intersecting arcs has a common intersection. The Proper Helly Circular-arc Vertex Deletion problem takes as input a graph $G$ and an integer $k$, and the goal is to check if we can remove at most $k$ vertices from the graph to obtain a proper Helly circular-arc graph; the parameter is $k$. Recently, Cao et al.~[MFCS 2023] obtained an FPT algorithm for this (and related) problem. In this work, we obtain a polynomial kernel for the problem.

==> preamble.tex <==
\usepackage{amsmath}
\usepackage[ruled,vlined,linesnumbered]{algorithm2e}%algopart %algosection %algochapter %algosection
\usepackage{adjustbox}

\usepackage{verbatim}
\usepackage{enumerate}
\usepackage{amssymb}
\usepackage{todonotes}
\usepackage{algpseudocode}
\usepackage{graphicx}
\usepackage{textcomp}
%\usepackage{algorithm}
\usepackage{epsfig}
\usepackage{amsfonts}
\usepackage{todonotes}
\usepackage[inline]{enumitem}
\usepackage{longtable}
\usepackage{xspace}
\usepackage{url}
\usepackage{latexsym}
\usepackage{amsmath}
\usepackage{verbatim}
\usepackage{enumerate}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{todonotes}
\usepackage{algpseudocode}
\usepackage{graphicx}
\usepackage{textcomp}
%\usepackage{algorithm}
\usepackage{epsfig}
\usepackage{amsfonts}
\usepackage{todonotes}
\usepackage[inline]{enumitem}
\usepackage{longtable}
\usepackage{xspace}
\usepackage{url}
\usepackage{tabularx}
%\usepackage{hyperref}
\let\proof\relax
\let\endproof\relax
\usepackage{amsthm}
\usepackage{thm-restate}
%\usepackage[dvipsnames]{xcolor}

%\usepackage{xcolor}
\usepackage{color, colortbl}
\definecolor{LRed}{rgb}{1,.8,.8}
\definecolor{MRed}{rgb}{1,.6,.6}
\definecolor{HRed}{rgb}{1,.2,.2}

%\usepackage[table,x11names]{xcolor}

\newcommand*{\field}[1]{\mathbb{#1}}%
\renewcommand{\labelitemi}{$\bullet$}
\newcommand{\tw}{{\sf tw}}
\newcommand{\pw}{{\sf pw}}

\DeclareMathAlphabet{\w}{OT1}{pzc}{m}{it}
\DeclareMathOperator{\ED}{\mathbb{E}_{\mathcal{D}}}
\newcommand{\card}[1]{\ensuremath{{\vert {#1} \vert }}}
%\newcommand{\C}[1]{\ensuremath{\operatorname{\mathcal {#1} }}}
\newcommand{\dmapsto}{\mathbin{\rotatebox[origin=c]{-90}{$\mapsto$}}}
\newcommand{\fn}[3]{\ensuremath{{{#1} : {#2} \rightarrow {#3}}}}
\newcommand{\zo}{\ensuremath{{\{0,1\}}}}
\newcommand{\set}[1]{\ensuremath{\left\{ {#1} \right\}}}
\newcommand{\ceil}[1]{\ensuremath{\left\lceil {#1} \right\rceil}}
\newcommand{\Ob}[1]{\ensuremath{\Omega\left({#1}\right)}}
\newcommand{\Lb}[1]{\ensuremath{\left({#1}\right)}}
\newcommand{\Sb}[1]{\ensuremath{\left[{#1}\right]}}
\newcommand{\mdsfull}{{\sc Mixed Dominating Set}\xspace}
\newcommand{\scfull}{{\sc Set Cover}\xspace}
\newcommand{\mds}{{\sc MDS}\xspace}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\npc}{\textsc{NP}-complete\xspace}
%\newcommand{\A}{\mathcal{A}}
\newcommand{\ppt}{\textsc{PPT}}
\newcommand{\rbds}{{\sc RBDS}}
\newcommand{\falgruntime}{{\OO((e\Delta(G))^k  \ell \vert A(G)\vert^2 \log  \vert A(G)\vert )}\xspace}
\newcommand{\fptruntimek}{{\OO^\star(7.465^k)}\xspace}
\newcommand{\fptruntimetw}{{\OO^\star(6^{\tw(G)})}\xspace}
\newcommand{\fptruntimekabs}{{7.465^k n^{\cO(1)}}\xspace}
\newcommand{\fptruntimetwabs}{{6^{\tw(G)} n^{\cO(1)}}\xspace}
\newcommand{\classP} {{\sf P}\xspace}
\newcommand{\tl}[1]{\ensuremath{\widetilde{{#1}}}}


\newcommand{\F}{{\mathcal F}}
%\newcommand{\S}{{\mathcal S}}
\newcommand{\T}{{\mathcal T}}

%\newcommand{\sC}{{\mathscr C}}
\newcommand{\OO}{{\mathcal O}}
\newcommand{\Yes}{{\sf Yes}}
\newcommand{\No}{{\sf No}}
\newcommand{\TDM} {{\sc $3$-Dimensional Matching}\xspace}
%\newcommand{\FPT} {{\sf FPT}\xspace}
\newcommand{\NPH} {{\sf NP}-hard\xspace}
%\newcommand{\NPC} {{\sf NP}-complete\xspace}
\newcommand{\WOH} {{\sf W}$[1]$-hard\xspace}
\newcommand{\WOHt} {{\sf W}$[2]$-hard\xspace}
\newcommand{\nokernelas} {{\sf coNP} $ \subseteq {\sf NP / poly}$}
\newtheorem{obs}{Observation}
\newcommand{\rbdsfull}{{\sc Red-Blue Dominating Set}}

\newtheorem{thm}{Theorem}
\newtheorem{theorem}{Theorem}
\newtheorem{observation}[thm]{Observation}
\newtheorem{definition}[thm]{Definition}
\newtheorem{lemma}[thm]{Lemma}
\newtheorem{proposition}[thm]{Proposition}
\newtheorem{claim}[thm]{Claim}
\newtheorem{corollary}[thm]{Corollary}
\newtheorem{remark}[thm]{Remark}

%\newtheorem{proposition}{Proposition}
%%%%%macros for dp
\newcommand{\fee}[1]{\ensuremath{F_{{#1}}}}
\newcommand{\pee}[1]{\ensuremath{P_{{#1}}}}
\newcommand{\vs}[1]{\ensuremath{Y_{{#1}}}}
\newcommand{\vnps}[1]{\ensuremath{N_{{#1}}}}
\newcommand{\vtdf}[1]{\ensuremath{T_{{#1}}}}
%%%%%%%%%%

 \newcommand{\defparproblem}[4]{
%  \vspace{1mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
   \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1  & {\bf{Parameter:}} #3
 \\ \end{tabular*}
% #1\\
  {\bf{Input:}} #2  \\
%  {\bf{Parameter:}} #3\\
  {\bf{Question:}} #4
  \end{minipage}
  }
 \vspace{1mm}
}


 \newcommand{\defparproblemnew}[5]{
%  \vspace{1mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
#1\\
  {\bf{Input:}} #2  \\
 {\bf{Parameter:}} #3\\
 {\bf{Parameter:}} #4\\
  {\bf{Question:}} #5
  \end{minipage}
  }
 \vspace{1mm}
}

 \newcommand{\defproblem}[3]{
%  \vspace{1mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
   \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1  %& {\bf{Parameter:}} #3
 \\ \end{tabular*}
% #1\\
  {\bf{Input:}} #2  \\
%  {\bf{Parameter:}} #3\\
  {\bf{Question:}} #3
  \end{minipage}
  }
 \vspace{1mm}
}


\newcommand{\ma}[1]{\todo[color={green!60!blue!20}]{\footnotesize{#1}}}

%\newcommand{\ma}[1]{\todo[color={green!50}]{#1}}

\newcommand{\sg}[1]{\todo[inline, color={green!50!blue!20}]{#1}}

\newcommand{\Note}[1]{\todo[inline, color={SpringGreen}]{\BrownB{NOTE :} {#1}}} 





%%%%%%%%dynamic parameterization %%%%%%%%%%%%%%%%%%%%%%%%


\usepackage{tikz}
\usetikzlibrary{positioning}
\usetikzlibrary{arrows}
\usetikzlibrary{shapes}
\usetikzlibrary{matrix}
\usepackage{graphicx}
\usepackage{microtype}%if unwanted, comment out or use option "draft"
\usepackage{complexity} % For symbols in complexity class.
\usepackage{threeparttable} 
%\usepackage[latin1]{inputenc}   
%\usepackage[T1]{fontenc}   
%\renewcommand{\M}{{\mathcal M}}


%%%%%%%%%%%%%%%%%%%%Cycle packing%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\usepackage{graphicx}
\usepackage{savesym}
\usepackage{amsmath, amssymb, amsthm,complexity}
%\usepackage{color}
\usepackage{pdfpages}
\usepackage{multirow}
%\usepackage[T1]{fontenc}
%\usepackage[utf8]{inputenc}
\usepackage{hyperref}

%\usepackage[utf8x]{inputenc}

\usepackage{amsmath,amssymb}
\usepackage{enumerate}

\usepackage{xspace}
%\usepackage{scrextend}

\usepackage{pfnote}

\usepackage{graphicx}
\usepackage{pdfpages}
%added by RK....end

\usepackage{authblk}
\usepackage{savesym}

\usepackage{amsmath, amssymb, complexity}



%%%%%%%%%%%%%%%%%%%%%%%%%%%This library redefining algorithms%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage{algorithmic}








\usepackage{comment}
%\usepackage{tempora}  % Times for numbers in math mode
\usepackage{thmtools}
\usepackage{thm-restate}
\usepackage{hyperref}

\usepackage{cleveref}
\usepackage{tikz}
\usetikzlibrary{shapes}
\usetikzlibrary{plotmarks}


%\usetikzlibrary{arrows.meta}

%\usepackage{verbatim}
%\usepackage[active,tightpage]{preview}
%\PreviewEnvironment{tikzpicture}
%\setlength\PreviewBorder{5pt}%
\usetikzlibrary{arrows,calc,shapes,decorations.pathreplacing}

\usepackage{wrapfig}
\usepackage{lscape}
\usepackage{rotating}
\usepackage{epstopdf}

\usepackage{pdfpages}

\newcommand{\alg}[1]{\mbox{\sf #1}} 
\newcommand{\algsub}[1]{\mbox{\sf\scriptsize #1}}

\usepackage{microtype}%if unwanted, comment out or use option "draft"

%\graphicspath{{./graphics/}}%helpful if your graphic files are in another directory
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\img}{img}
\DeclareMathOperator{\paths}{paths}



%%%%%%%%%%%%%%%%%%%%%%%Cycles in tournaments$$$$$$$$$$$$$$$$$$$$$$$$$$$$$$$$$$$$$$$$$$$$

\usepackage{amsmath, amssymb, amsthm}%,complexity}
\renewcommand{\W}{{\sf W}}
\renewcommand{\XP}{{\sf XP}}

\usepackage{pdfpages}


\usepackage{todonotes}
\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
%\usepackage{algorithmic}
\usepackage{comment}

\usepackage{thmtools}
\usepackage{thm-restate}
\usepackage{hyperref}

\usepackage{cleveref}
\usepackage{tikz}
\usepackage{amsmath}
\usetikzlibrary{shapes}
\usetikzlibrary{plotmarks}
%\usetikzlibrary{arrows.meta}

%\usepackage{verbatim}
%\usepackage[active,tightpage]{preview}
%\PreviewEnvironment{tikzpicture}
%\setlength\PreviewBorder{5pt}%
\usetikzlibrary{arrows,calc,shapes,decorations.pathreplacing}

\usepackage{wrapfig}
\usepackage{lscape}
\usepackage{rotating}
\usepackage{epstopdf}

\renewcommand{\alg}[1]{\mbox{\sf #1}}
\renewcommand{\algsub}[1]{\mbox{\sf\scriptsize #1}}


%\theoremstyle{definition}
%
\theoremstyle{plain}
%\newtheorem{proposition}[theorem]{Proposition}%[section]
%\newtheorem{observation}[theorem]{Observation}%[section]
%\declaretheorem[name=Theorem]{thm}

\newtheorem{reduction rule}{Reduction Rule}[section]



%\newcommand{\cpt}{\textsc{Arc-Disjoint Cycle Packing in Tournaments}}
%\newcommand{\cp}{\textsc{Arc-Disjoint Cycle Packing}}
%\newcommand{\vcp}{\textsc{Vertex-Disjoint Cycle Packing}}

\newcommand{\act}{\textsc{ACT}}
\newcommand{\att}{\textsc{ATT}}

\newcommand{\sat}{{\sc SAT}}

\newcommand{\fast}{\textsc{FAST}}
\newcommand{\oo}{\mathcal{O}}
\newcommand{\ostar}{\mathcal{O}^\star}
\newcommand{\mc}{\mathcal{C}}
\newcommand{\mf}{\mathcal{F}}
\newcommand{\ms}{\mathcal{S}}
\newcommand{\mi}{\mathcal{I}}
\newcommand{\mj}{\mathcal{J}}

%\DeclareMathOperator{\dom}{dom}
%\DeclareMathOperator{\img}{img}
%\DeclareMathOperator{\paths}{paths}
\DeclareMathOperator{\fas}{minfas}
\DeclareMathOperator{\first}{first}
\DeclareMathOperator{\second}{mid}
\DeclareMathOperator{\head}{h}
\DeclareMathOperator{\tail}{t}

\makeatletter
\newcommand{\injective}[2][]{\ext@arrow 0359\rightarrowfill@{#1}{#2}}
\makeatother

\newcommand{\defparprob}[4]{
  \vspace{2mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} \textsc{#1}  & {\bf{Parameter:}} #3
\\ \end{tabular*}
  {\bf{Input:}} #2  \\
  {\bf{Question:}} #4
  \end{minipage}
  }
  \vspace{2mm}
}

\newcommand{\defparprobopt}[5]{
  \vspace{2mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} \textsc{#1}  & {\bf{Parameter:}} #3
\\ \end{tabular*}
  {\bf{Instance:}} #2  \\
  {\bf{Feasible Solution:}} #4
  {\bf{Optimum Solution:}} #5
  \end{minipage}
  }
  \vspace{2mm}
}

%%%%% Packages and Commands:KSSZ:end


%%%%% Packages and Commands:BBT:start

%-------------------------------------------%

%\usepackage{authblk}% affiliation   %Commented by RK
\usepackage{amssymb,amsmath,amsthm}
\usepackage{float}
\usepackage{changepage}
\usepackage{enumerate} % lists with (i), (ii), (iii), ...
\usepackage{tikz}
\usepackage{thmtools} % autoref
\usepackage{hyperref, cleveref} %autoref
\usepackage{breqn} %multiple line equations
%\usepackage{showlabels}

%-------------------------------------------%
%%%Commented by RK -start
%\textwidth 16cm
%\textheight 21cm
%\evensidemargin 0cm
%\oddsidemargin 0cm
%%%Commented by RK -end
%-------------------------------------------%

\newcommand{\ra}{\rightarrow}


%-------------------------------------------%

%%%Commented by RK -start

\theoremstyle{plain}
%\newtheorem{theorem}{Theorem}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{claim}{Claim}[theorem]
%\newtheorem{observation}[theorem]{Observation}

%%%Commented by RK -end

%% PROBLEM DEFINITION COMMAND
\newcommand{\data}{\textbf{Input: }}
\newcommand{\quest}{\textbf{Output: }}
\newcommand{\res}{\textbf{Result: }}
\newcommand{\opt}{\textbf{Optimization: }}
\newenvironment{oproblem}[4]{\begin{figure}[H]\begin{adjustwidth}{0.5cm}{}{\sc#1}\\ \data #2\\ \res #3\\ \opt #4}{\end{adjustwidth}\end{figure}\vspace{-1em}}
\newenvironment{qproblem}[3]{\begin{figure}[H]\begin{adjustwidth}{0.5cm}{}{\sc#1}\\ \data #2\\ \quest #3}{\end{adjustwidth}\end{figure}\vspace{-1em}}


%-------------------------------------------%

%\newcommand{\x}{X}
\newcommand{\xalpha}{|\bA{A}^{vc}(\T)|}
\newcommand{\x}{\mathcal{X}}
\newcommand{\tx}{\tilde{\x}}
\newcommand{\Vx}{V_\x}
\newcommand{\Ax}{A_\x}
\newcommand{\B}{B}
\renewcommand{\p}{U}
\renewcommand{\M}{M}
\newcommand{\Ap}{A'}
\newcommand{\Apb}{\overline{\Ap}}
\newcommand{\Up}{U'}
\newcommand{\Upb}{\overline{\Up}}
\newcommand{\Uf}{\p[F]}

\newcommand{\ord}{\sigma}
\newcommand{\lo}{<_\ord}
\newcommand{\ba}{b}
\newcommand{\Gf}{G'}
\newcommand{\Vf}{V'}
\newcommand{\Af}{A'}
%\newcommand{\T}{{\cal T}}
\renewcommand{\T}{{T}}
\newcommand{\V}{\sigma}
\newcommand{\Pip}{\Pi'}

\renewcommand{\t}{\delta}

\renewcommand{\S}{\Delta}
\renewcommand{\SC}{O}
\newcommand{\Tv}{T_{v}}
\newcommand{\Tc}{T_{c}}
\newcommand{\Vv}{\V}
\newcommand{\Vc}{\V}
\newcommand{\Vcv}{\V^{cv}}
\newcommand{\SVVV}{\S_{V,V,V}}
\newcommand{\SVVC}{\S_{V,V,C}}
\newcommand{\SVCC}{\S_{V,C,C}}
\newcommand{\SCCC}{\S_{C,C,C}}
\newcommand{\SdVC}{\S_{2V,C}}
\newcommand{\SVdC}{\S_{V,2C}}
\newcommand{\StV}{\S_{3V}}
\newcommand{\StC}{\S_{3C}}

\newcommand{\So}{\S}
\newcommand{\SoVVV}{\So_{V,V,V}}
\newcommand{\SoVVC}{\So_{V,V,C}}
\newcommand{\SoVCC}{\So_{V,C,C}}
\newcommand{\SoCCC}{\So_{C,C,C}}
\newcommand{\SodVC}{\So_{2V,C}}
\newcommand{\SoVdC}{\So_{V,2C}}
\newcommand{\SodCC}{\So_{2C,C}}
\newcommand{\SoCdC}{\So_{C,2C}}
\newcommand{\SotV}{\So_{3V}}
\newcommand{\SotC}{\So_{3C}}
\newcommand{\Sv}{\S^{v}}
\newcommand{\SVVVp}{\Sv_{V,V,V}}
\newcommand{\Sc}{\S^{c}}
\newcommand{\SCCCp}{\Sc_{C,C,C}}

\newcommand{\CVV}{\SC_{V^*}}
\newcommand{\CV}{\SC_{V}}
\newcommand{\CCC}{\SC_{C^*}}
\newcommand{\CC}{\SC_{C}}
\newcommand{\CVC}{\SC_{V^*,C^*}}


%%% PROBLEM NOTATIONS

\newcommand{\cpt}{\textsc{Arc-Disjoint Cycle Packing in Tournaments}}
\newcommand{\cp}{\textsc{Arc-Disjoint Cycle Packing}}
\newcommand{\vcp}{\textsc{Vertex-Disjoint Cycle Packing}}




%\newcommand{\maxtst}{{\sc ATST}} % triangle packing on sparse tournaments
%\newcommand{\maxcst}{{\sc ACST}} % cycle packing on sparse tournaments

%\newcommand{\maxtst}{{\sc MaxTST}} % triangle packing on sparse tournaments
%\newcommand{\maxcst}{{\sc MaxCST}} % cycle packing on sparse tournaments

%\newcommand{\kmaxtst}{$k$-\maxtst} % parameterized triangle packing on sparse tournaments

%\newcommand{\maxtt}{{\sc ATT}} % triangle packing on tournaments
%\newcommand{\kmaxtt}{$k$-\maxtt}% parameterized triangle packing on tournaments

\newcommand{\maxtt}{{\sc MaxATT}} % triangle packing on tournaments
\newcommand{\kmaxtt}{{\sc ATT}}% parameterized triangle packing on tournaments

%\newcommand{\maxct}{{\sc ACT}} % cycle packing on tournaments
%\newcommand{\kmaxct}{$k$-\maxct} % parameterized cycle packing on tournaments
%Changed by RK
\newcommand{\maxct}{{\sc MaxACT}} % cycle packing on tournaments
\newcommand{\kmaxct}{{\sc ACT}} % parameterized cycle packing on tournaments

%\newcommand{\maxtttight}{{\sc Tight-\maxtt}}
%\newcommand{\maxcttight}{{\sc Tight-\maxct}}

\newcommand{\maxtttight}{{\sc Tight-\att}}
\newcommand{\maxcttight}{{\sc Tight-\act}}


\newcommand{\tsatt}{{\sc 3-SAT(3)}}
\newcommand{\tdm}{{\sc 3-Dimensional Matching}}

%%% COMPLEXITY NOTATIONS
\renewcommand{\NP}{{\sf NP}}
\renewcommand{\P}{{\sf P}}
\renewcommand{\coNP}{co\NP/poly}
\renewcommand{\PTAS}{{\sf PTAS}}
\renewcommand{\FPT}{{\sf FPT}}
\renewcommand{\APX}{{\sf APX}}


%%% BACKWARD/FORWARD ARCS NOTATION
\renewcommand{\A}{A}
\newlength{\mylfA}
\newlength{\myhfA}

\newcommand{\fA}[1]{%
\settowidth{\mylfA}{#1}
\def\sizefB{\the\mylfA}
\settoheight{\myhfA}{#1}
\def\heightfB{\the\myhfA}
\hspace{-0.35em}
\begin{tikzpicture}[baseline=(O.base)]
\draw[ -> ](0,\heightfB)  -- ( \sizefB, \heightfB);
\node (O) at (\sizefB/2,\heightfB/7-0.01ex) {$#1$};
\end{tikzpicture}%
\hspace{-0.35em}
}

\newcommand{\bA}[1]{%
\settowidth{\mylfA}{#1}
\def\sizefB{\the\mylfA}
\settoheight{\myhfA}{#1}
\def\heightfB{\the\myhfA}
\hspace{-0.35em}
\begin{tikzpicture}[baseline=(O.base)]
\draw[ <- ](0,\heightfB)  -- ( \sizefB, \heightfB);
\node (O) at (\sizefB/2,\heightfB/7-0.01ex) {$#1$};
\end{tikzpicture}%
\hspace{-0.35em}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%cycle path cover%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\documentclass[envcountsame,10pt]{llncs}
%\documentclass[runningheads]{llncs}
%added by RK...start
\usepackage{float}
\usepackage{graphicx}
\usepackage{complexity}
%\usepackage{amssymb}
\usepackage{savesym}
%\usepackage{amsmath}
%\usepackage{color}
\usepackage{pdfpages}
%\savesymbol{vec}
%\usepackage{euler}
%\restoresymbol{eul}{vec}

\usepackage{tcolorbox}
\tcbuselibrary{skins,breakable}

%\DeclareMathOperator{\conv}{conv}
%\mathchardef\hyphen="2D
\newenvironment{lemma-l}[1]{\noindent {\bf Lemma~#1.~}\em }{\smallskip}
\newenvironment{theorem-t}[1]{\noindent {\bf Theorem~#1.~}\em }{\smallskip}
%\newtheorem{observation}[theorem]{Observation}
\renewcommand{\thefootnote}{\fnsymbol{footnote}}
%\usepackage{perpage}
%\MakePerPage{footnote}
%\renewcommand{\rmdefault}{ppl} % rm
%\linespread{1.05}        % Palatino needs more leading
%\usepackage[scaled]{helvet} % ss
%\usepackage{courier} 
% tt
%\usepackage{euler} % math %\usepackage{eulervm} % a better implementation of the euler package (not in gwTeX)
%\normalfont

\pagestyle{plain}

%\usepackage[T1]{fontenc}
%%%%%%
%\pagestyle{plain}

%%%%%%%%%%% HERE IT STARTS %%%%%%%%%%%%%%%%%%%%%%%%%%

%\documentclass[a4paper,10pt]{article}

%\documentclass[svgnames,dvipsnames,nofootinbib]{llncs}
%\usepackage{microtype}
\usepackage{multirow}
%\usepackage[T1]{fontenc}
%\usepackage[utf8]{inputenc}
\usepackage{hyperref}

%\usepackage[utf8x]{inputenc}

\usepackage{amsmath,amssymb}
%\newtheorem{definition}{Definition}
%\newtheorem{proposition}{Proposition}
%\newtheorem{lemma}{Lemma}
%\newtheorem{theorem}{Theorem}
%\newtheorem{claim}{Claim}
%\newtheorem{observation}{Observation}
%\newtheorem{corollary}{Corollary}
\newtheorem{Reduction Rule}{Reduction Rule}
%\usepackage{fullpage}
%\usepackage{mathtools}
%\usepackage{showframe}
%\usepackage{hyperref}
%\newcommand{\lemmaautorefname}{Lemma}
\newcommand\Myperm[2][n]{\prescript{#1\mkern-2.5mu}{}P_{#2}}
\newcommand\Mycomb[2][n]{\prescript{#1\mkern-0.5mu}{}C_{#2}}
\usepackage{enumerate}

\usepackage{xspace}
%\usepackage{scrextend}

\usepackage{pfnote}

\usepackage{graphicx}
\usepackage{pdfpages}
%added by RK....end


\usepackage{savesym}

\usepackage{amsmath, amssymb, complexity}
\usepackage{todonotes}
\usepackage[ruled,vlined,linesnumbered]{algorithm2e}%algopart %algosection %algochapter %algosection
%\usepackage{algorithmic}
\usepackage{comment}
%\usepackage{tempora}  % Times for numbers in math mode
\usepackage{thmtools}
\usepackage{thm-restate}
\usepackage{hyperref}

\usepackage{cleveref}
\usepackage{tikz}
\usetikzlibrary{shapes}
\usetikzlibrary{plotmarks}


%\usetikzlibrary{arrows.meta}

%\usepackage{verbatim}
%\usepackage[active,tightpage]{preview}
%\PreviewEnvironment{tikzpicture}
%\setlength\PreviewBorder{5pt}%
\usetikzlibrary{arrows,calc,shapes,decorations.pathreplacing}

\usepackage{wrapfig}
\usepackage{lscape}
\usepackage{rotating}
\usepackage{epstopdf}

\usepackage{pdfpages}
\usepackage{amsmath, amssymb}%, amsthm}%,complexity}
%\newcommand{\W}{{\sf W}}
%\newcommand{\XP}{{\sf XP}}
\usepackage{framed}

\usepackage{pdfpages}


\usepackage{todonotes}
%\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
%\usepackage{algorithmic}
\usepackage{comment}

\usepackage{thmtools}
\usepackage{thm-restate}
\usepackage{hyperref}

\usepackage{cleveref}
\usepackage{tikz}
\usepackage{amsmath}
\usetikzlibrary{shapes}
\usetikzlibrary{plotmarks}
%\usetikzlibrary{arrows.meta}

%\usepackage{verbatim}
%\usepackage[active,tightpage]{preview}
%\PreviewEnvironment{tikzpicture}
%\setlength\PreviewBorder{5pt}%
\usetikzlibrary{arrows,calc,shapes,decorations.pathreplacing}

\usepackage{wrapfig}
\usepackage{lscape}
\usepackage{rotating}
\usepackage{epstopdf}

\renewcommand{\alg}[1]{\mbox{\sf #1}} 
\renewcommand{\algsub}[1]{\mbox{\sf\scriptsize #1}}


%\theoremstyle{definition}
%
%\theoremstyle{plain}
%\newtheorem{proposition}[theorem]{Proposition}%[section]
%\declaretheorem[name=Theorem]{thm}

%\newtheorem{reduction rule}{Reduction Rule}[section]
%\newtheorem{observation}[theorem]{Observation}%[section]




\renewcommand{\oo}{\mathcal{O}}
\renewcommand{\ostar}{\mathcal{O}^\star}
%\newcommand{\mc}{\mathcal}
\renewcommand{\mf}{\mathcal{F}}
\renewcommand{\ms}{\mathcal{S}}
\renewcommand{\mi}{\mathcal{I}}
\renewcommand{\mj}{\mathcal{J}}

%\DeclareMathOperator{\dom}{dom}
%\DeclareMathOperator{\img}{img}
%\DeclareMathOperator{\paths}{paths}
%\DeclareMathOperator{\fas}{minfas}
%\DeclareMathOperator{\first}{first}
%\DeclareMathOperator{\second}{mid}
%\DeclareMathOperator{\head}{h}
%\DeclareMathOperator{\tail}{t}

%\makeatletter
%\newcommand{\injective}[2][]{\ext@arrow 0359\rightarrowfill@{#1}{#2}}
%\makeatother

\renewcommand{\defparprob}[4]{
  \vspace{2mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} \textsc{#1}  & {\bf{Parameter:}} #3
\\ \end{tabular*}
  {\bf{Input:}} #2  \\
  {\bf{Question:}} #4
  \end{minipage}
  }
  \vspace{2mm}
}

\renewcommand{\defparprobopt}[5]{
  \vspace{2mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} \textsc{#1}  & {\bf{Parameter:}} #3
\\ \end{tabular*}
  {\bf{Instance:}} #2  \\
  {\bf{Feasible Solution:}} #4
  {\bf{Optimum Solution:}} #5  
  \end{minipage}
  }
  \vspace{2mm}
}

%%%%% Packages and Commands:KSSZ:end



\newcommand{\lab}{\ell}


\usepackage{complexity}
\usepackage{graphicx,wrapfig,lipsum}

%\newcommand{\alg}[1]{\mbox{\sf #1}} 
%\newcommand{\algsub}[1]{\mbox{\sf\scriptsize #1}}

\usepackage{microtype}%if unwanted, comment out or use option "draft"

%\graphicspath{{./graphics/}}%helpful if your graphic files are in another directory

%\bibliographystyle{plainurl}% the recommended bibstyle
